Design by Contract Framework for Quantum Software

To realize reliable quantum software, techniques to automatically ensure the quantum software's correctness have recently been investigated. However, they primarily focus on fixed quantum circuits rather than the procedure of building quantum circuits. Despite being a common approach, the correctness of building circuits using different parameters following the same procedure is not guaranteed. To this end, we propose a design-by-contract framework for quantum software. Our framework provides a python-embedded language to write assertions on the input and output states of all quantum circuits built by certain procedures. Additionally, it provides a method to write assertions about the statistical processing of measurement results to ensure the procedure's correctness for obtaining the final result. These assertions are automatically checked using a quantum computer simulator. For evaluation, we implemented our framework and wrote assertions for some widely used quantum algorithms. Consequently, we found that our framework has sufficient expressive power to verify the whole procedure of quantum software.

==> existing_works.tex <==
\section{Existing Works}
\label{sec:existing_works}

Paykin et al. \cite{Paykin:qwire} developed the first verifiable quantum language
% implemented in Coq, 
and Hietala et al. \cite{Hietala:SQIR} improved it.
Liu \cite{liu2019:QHLProver} implemented quantum Hoare logic \cite{ying2012} in Isabell/HOS. 
% , which is an extension of Hoare logic \cite{hoare1969} to quantum computing.
These works can verify quantum software formally but be applied only to fixed-size quantum circuits.
Chareton et al. \cite{Chareton2021:Qbricks} proposed an (almost) automated formal verification tool for verifying quantum circuits whose features, such as size, gates, and count of repetitions, are parameterized. This tool can ensure the correctness of the procedures of building quantum circuits. However, the procedure is limited to appending gates, rendering gates reverted or controlled, and repeating.
Thus, this tool cannot verify complicated procedures for building quantum circuits.
Moreover, this tool lacks measurement operation and cannot write statistical processing of measurement results. % for obtaining the final result.

Huang and Martonosi \cite{huang2019} suggested adding assertions to quantum circuits and verifying them on quantum computers using statistics analysis.
The assertions that their framework can handle are restricted only to several types of quantum states.
% : whether the states of qubits are classical, the states of qubits are a superposition of some states, or specified qubits are entangled.
Liu et al.\cite{liu2020}  suggested a technique to examine the same type of assertions by measuring ancilla qubits to avoid destructing quantum states.
Li et al. \cite{li2020} suggested a projection-based technique to check runtime assertions.
In their framework, arbitrary quantum states can be expressed by projections.
These techniques are well-matched to run on quantum computers but can check only fixed quantum states.

% Ying \cite{ying2012} extended Hoare logic \cite{hoare1969} to quantum computing.
% It enables us to write pre-condition $P$ and post-condition $Q$ on a quantum program $S$ with a triple $\{P\}S\{Q\}$ and verify it by inference rules.

% Their logic can write any condition about the quantum states. However, automatic verification is challenging.


Some techniques use assertions about quantum states for automatic testing \cite{honarvar2020,wang2021,wang2022}.
% These techniques enable us to test automatically. 
However, they do not focus on the procedure of building quantum circuits.

Q\# \cite{qsharp} provides a feature to write assertions and check them in runtime.
However, the assertions are limited to measurement results, so the users cannot verify quantum states directly.

